Distributional Hamilton-Jacobi-Bellman Equations for Continuous-Time Reinforcement Learning

Continuous-time reinforcement learning offers an appealing formalism for describing control problems in which the passage of time is not naturally divided into discrete increments. Here we consider the problem of predicting the distribution of returns obtained by an agent interacting in a continuous-time, stochastic environment. Accurate return predictions have proven useful for determining optimal policies for risk-sensitive control, learning state representations, multiagent coordination, and more. We begin by establishing the distributional analogue of the Hamilton-Jacobi-Bellman (HJB) equation for It\^o diffusions and the broader class of Feller-Dynkin processes. We then specialize this equation to the setting in which the return distribution is approximated by $N$ uniformly-weighted particles, a common design choice in distributional algorithms. Our derivation highlights additional terms due to statistical diffusivity which arise from the proper handling of distributions in the continuous-time setting. Based on this, we propose a tractable algorithm for approximately solving the distributional HJB based on a JKO scheme, which can be implemented in an online control algorithm. We demonstrate the effectiveness of such an algorithm in a synthetic control problem.

==> rl.tex <==
\section{Reinforcement Learning}\label{s:rl}

Given the characterizations of the return distribution function illustrated in the previous
section, we shift our focus to the construction of RL algorithms for
learning the return distribution function for an agent evolving according to a Feller-Dynkin 
process. As in section \ref{s:dhjb:representation}, we concern ourselves mainly with the
setting in which the agent's dynamics are governed by an \Ito\ diffusion.

In Corollary \ref{cor:shjb}, we see that, under the quantile representation, the 
\emph{distributional} HJB equation is simply a system of PDEs having the same form as 
\eqref{eq:hjb}. As such, given an oracle $\hjbsolve$ for the HJB equation, we can construct a
continuous-time distributional RL algorithm by invoking $\hjbsolve$ for the HJB equations 
corresponding to each quantile. This procedure can naturally be cast as an optimization in the
space of probability measures. To conquer this challenge, we appeal to the celebrated minimizing
movements scheme of Jordan, Kinderlehrer, and Otto \citep{Jordan02thevariational} known as the 
\emph{JKO scheme}. Roughly, this amounts to optimizing an objective (in our case, proximity to 
a solution to the distributional HJB equation) with a 2-Wasserstein distance regularization term
that penalizes successive solution iterates from deviating too quickly. Since we cannot compute
2-Wasserstein gradients from samples \citep{bellemare2017cramer}, we instead approximate the
2-Wasserstein regularization via entropically regularised optimal transport 
\citep{cuturi2013sinkhorn}. Such an approximation is common in the machine learning literature. 
In particular, \citet{martin2020stochastically} makes the same 
approximation for learning the return distribution function. Implementation details
for such a continuous-time distributional RL algorithm are given in Appendix 
\ref{s:algorithms}.

The remainder of this section serves to demonstrate how the theoretical discrepancies of 
discrete-time reinforcement learning algorithms in the continuous-time setting 
manifest themselves in practice. To this end, we compare the performance of an algorithm that 
solves the  distributional HJB equation as discussed above with the established discrete-time 
QTD algorithm of \citet{Dabney2018DistributionalRL} facing a very simple MDP whose analytical
return distribution function can be readily computed and visualized. We will consider an MDP
inspired by a problem posed in \citet{Munos2004ASO}, which
has state space $\xxX = [0,1]$ and action space $\xxA = \{-1,1\}$, and the agent evolves
according to the dynamics $\frac{d}{dt}x(t) = \dot{x}(t)$ given by $\dot{x}(t) = a(t)$.
The rewards are zero everywhere in $(0,1)$, and are otherwise sampled from $\mathcal{N}(1,1)$
and $\mathcal{N}(2, 2)$ at $x=0$ and $x=1$ respectively. We discretize the evolution of the MDP
to timesteps of duration $10^{-3}$ and evaluate the return distributions learned by QTD and our
proposed algorithm, denoted CT-QTD\footnote{This refers to \emph{continuous-time} QTD.}, over
the state space. The results are shown in Figure \ref{fig:birdseye}.
\begin{figure}[h!]
  \centering
  \ifconfelse{icml2022}{%
  \newcommand{\dtscale}{0.226}
  \newcommand{\ctscale}{0.339}
  QTD\\
  \includegraphics[scale=\dtscale, trim={0 0 0 2cm},
  clip]{results/dt51-munos-overview}\\
  CT-QTD\\
  \includegraphics[scale=\ctscale, trim={0 0 0 1.5cm}, clip]{results/ct51-munos-overview-0}%
  }{%
  \newcommand{\dtscale}{0.21}
  \newcommand{\ctscale}{0.32}
  \begin{minipage}{0.495\textwidth}
  \centering
  QTD\\
  \includegraphics[scale=\dtscale, trim={0 0 0 2cm},
  clip]{results/dt51-munos-overview}\\
  \end{minipage}
  \begin{minipage}{0.495\textwidth}
  \centering
  CT-QTD\\
  \includegraphics[scale=\ctscale, trim={0 0 0 1.5cm}, clip]{results/ct51-munos-overview-0}%
  \end{minipage}
  }
  \caption{Return distribution functions and policies learned by QTD and a continuous-time counterpart}
  \label{fig:birdseye}
\end{figure}

Two notable observations should be made with regard to Figure \ref{fig:birdseye}. Firstly, we
see that QTD struggles to make proper variance estimates at states that are not in the immediate
vicinity of the rewarding states, while CT-QTD is able to propagate variance estimates across
the state space. Moreover, we see that even the mean of the return distributions is not 
accurately learned by QTD. The discrepancy appears to stem from the point of 
non-differentiability of the analytical value function, and consequently the value function
extracted from QTD's return distribution function is not a \emph{viscosity solution} 
\citep{crandall1983viscosity} -- which is precisely the failure mode of discrete-time RL
predicted by \citet{Munos2004ASO}. On the other hand, it is clear that the mean return
(value) function learned by CT-QTD \emph{is} a viscosity solution, and adheres quite well to the
analytical value function.

From these observations, we may conclude that continuous-time considerations may produce 
tangible benefits for distributional RL, even in exceptionally simple MDPs. This illustrates
the importance of analyzing distributional RL in the continuous-time setting.
